End-to-End Incremental Learning

Although deep learning approaches have stood out in recent years due to their state-of-the-art results, they continue to suffer from catastrophic forgetting, a dramatic decrease in overall performance when training with new classes added incrementally. This is due to current neural network architectures requiring the entire dataset, consisting of all the samples from the old as well as the new classes, to update the model -a requirement that becomes easily unsustainable as the number of classes grows. We address this issue with our approach to learn deep neural networks incrementally, using new data and only a small exemplar set corresponding to samples from the old classes. This is based on a loss composed of a distillation measure to retain the knowledge acquired from the old classes, and a cross-entropy loss to learn the new classes. Our incremental training is achieved while keeping the entire framework end-to-end, i.e., learning the data representation and the classifier jointly, unlike recent methods with no such guarantees. We evaluate our method extensively on the CIFAR-100 and ImageNet (ILSVRC 2012) image classification datasets, and show state-of-the-art performance.

==> extratext.tex <==

%%relwork.tex

%Similar to iCaRL, the gradient episodic memory (GEM) model~\cite{lopez2017nips} stores an exemplar set (referred to as episodic memory) to maintain the performance on the old classes. While iCaRL uses a distillation loss to reduce catastrophic forgetting, GEM solves a quadratic program with inequality constraints ensuring that the loss of the model updated with new data is no greater than the one computed with the previous model. GEM shows slightly better performance than iCaRL on CIFAR100, but ...



%%method.tex

%We borrow from~\cite{rebuffi2017cvpr}, the idea of keeping a limited subset of training samples to reinforce the knowledge from classes previously trained. By this way, the deep model has some representative samples from each class to keep its behaviour and, at the same time, to learn how to build a new representation and a classifier to separate old and new classes. This subset of samples is stored and managed by the representative memory.

%The second part is the deep model which can be any model designed for classification, since our approach does not require any specific characteristic. The only necessary modification is a specific loss function which is described in Sec.~\ref{sec:deep_model}.

%In the next subsections, we describe in detail the two main components commented above.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[tb]
%    \centering
%    \includegraphics[width=0.99\textwidth]{./images/model_basic.pdf}
%    \caption{\textbf{Incremental learning}. Every classification layer takes  features from the feature extractor to produce a set of \textit{logits}. All these \textit{logits} are combined in the softmax layer to produce a global probability distribution.}
%    \afterCaption
%    \label{fig:model2}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%method.tex
%\myparagraph{Selection of new samples}. The selection of the samples is based on \textit{herding}~\cite{welling2009icml}. This selection keeps a set of samples of one class whose mean is close to the mean of the whole training set of that class. Therefore, the stored set of samples of one class is a sorted list where the first sample contributes more to a closer mean than the last sample. \new{Given the} sorted list of samples, it stores the first $n$ samples of the list which are the most representative samples of the class according to the mean.
%During the training of new classes, this set of representative samples helps the deep model to approximate the representation of one class to its mean. In addition, although the number of samples per class is low, the stored samples would represent the best mean possible for that number of samples.



%%method.tex
%After this first execution, the samples are stored in a sorted way and if we need to release memory for new classes, the memory only has to remove samples from the end of the list. 



%%method.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[tb]
%    \centering
%    \includegraphics[width=0.47\textwidth]{./images/model.pdf}
%    \caption{\textbf{Incremental architecture}. Every classification layer takes  features from the feature extractor to produce a set of logits. All these logits are combined in the global softmax layer to produce a global probability distribution.}
%    \afterCaption
%    \label{fig:model}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%method.tex
%The distillation loss function $L_{D}(\omega)$, shown in Eq.~\ref{eq:distillation_loss}, looks like a traditional cross-entropy function but using a modified version of $p_i$ and $q_i$: $pdist_i$ and $qdist_i$, respectively. These modified versions are obtained by raising $p_i$ and $q_i$ to the exponent $1/T$ as described in~\cite{hinton2014nips}. In this case, $T$ is the distillation parameter. If $T>1$, it increases the weight of smaller \textit{logit} values and reinforce the learning of similarities between classes. Preliminary experiments showed that best results were obtained for a value of $T=2$. Hence, we set $T$ to 2 for all our experiments.

%The clarify the differences between $L_{C}(\omega)$ and $L_{D}(\omega)$ and their effect in the output probabilities, Fig.~\ref{fig:activations} shows the output probabilities of one sample for a classification layer trained with a cross-entropy loss (Fig.~\ref{fig:activations}a) and the same classification layer trained with the distillation loss (Fig.~\ref{fig:activations}b). The effect is evident, while in a), there is a big peak in the activations, in b), the peak is softer and the probabilities are distributed across the classes . This effect is useful to retain the knowledge because this distributed probability means that the weights in the network are more interrelated between them. Therefore, to produce an output, more parts of the network play an important role and the final model is more robust and small changes in the weights (produced by the training of the new classes) produce similar results. 
%To sum up, we propose a new loss function designed for incremental learning. This loss combines in a new way two well known functions such as cross-entropy loss and distillation loss, used for classification and network compression respectively.

%Our cross-distilled loss function combines a distillation loss~\cite{hinton2014nips} used to retain the knowledge from old classes with a cross-entropy loss for classification. Therefore, this distillation loss function only produces gradients on the \textit{classification layers} of the old classes. On the other hand, the cross-entropy loss is used both for training the \textit{classification layer} for the new classes and for reinforcing the separability of old and new classes. 

%We use as distillation loss the function proposed by Hinton \etal~\cite{hinton2014nips}, which is a modified cross-entropy that increases the weights of the small probabilities. Therefore, after training the model with this loss function, the probabilities produced by the \textit{classification layers} of the old classes are more distributed between all outputs of the layer than in a classification layer trained only with a traditional cross-entropy layer. This effect can be seen in Fig.~\ref{fig:activations}, where the left plot represents the output probabilities of a sample obtained from a \textit{classification layer} with ten classes after being trained with a cross-entropy loss (its classes are new classes). Right plot represents the probabilities of the same \textit{classification layer} after being trained with distillation loss (its classes are now old classes). Thus, due to this behaviour, when the outputs of the global softmax layer are collected, most of the times, the highest probabilities will be focused on the new classes and the accuracy will drop.  This problem is mitigated with our cross-entropy loss connected to \textit{classification layers} for old and new classes because it helps to the classifiers to scale their outputs for being in a similar range. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[tb]
%    \centering
%    \includegraphics[width=0.8\textwidth]{./images/activations.pdf}
%    \caption{\textbf{Probability distributions}. (a) The output probabilities of a sample obtained from a classification layer trained with cross-entropy loss function (Eq.~\ref{eq:cross-entropy}). (b) The probabilities of the same classification layer after being trained with distillation loss (Eq.~\ref{eq:distillation_loss}). More details in the main text.}
%    \afterCaption
%    \label{fig:activations}
%\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Let $q_i$ be a prediction obtained from the \textit{classification layer}, $p_i$ the ground-truth for that sample, and $\omega$ the weights of the model, the cross-entropy function is defined as:
%\beforeEquation
%\begin{equation}\label{eq:cross-entropy}
%    L_{C}(\omega) = -\frac{1}{N} \sum_{i=1}^{N} \sum_{j=1}^{C} p_{ij} \log q_{ij},
%\afterEquation
%\end{equation}
%where $N$ is the total number of samples and $C$ the total number of classes.

%For our distillation loss, we need to recompute $p_i$ and $q_i$ following the indications in~\cite{hinton2014nips}. The modified versions are defined as:
%\beforeEquation
%\begin{equation}
%    pdist_i = \frac{p_i^{1/T}}{\sum_j p_j^{1/T}},
%    \qquad
%    qdist_i = \frac{q_i^{1/T}}{\sum_j q_j^{1/T}},
%\afterEquation
%\end{equation}
%where $T$ is distillation parameter. If $T>1$, it increases the weight of smaller \textit{logit} values %and reinforce the learning of similarities between classes.

%After these modifications, the distillation loss function looks like a traditional cross-entropy %function but using the modified versions of $p_i$ and $q_i$: $pdist_i$ and $qdist_i$ respectively:
%\beforeEquation
%\begin{equation}
%    L_{D}(\omega) = -\frac{1}{N} \sum_{n=1}^{N} \sum_{j=1}^{C} pdist_{ij} \log qdist_{ij},
%\afterEquation
%\end{equation}
%where $N$ is the total number of samples and $C$ the total number of classes.

%Finally, our combined loss function is defined as:
%\beforeEquation
%\begin{equation}
%    L(\omega) = L_{C}(\omega) + \sum_{f=1}^{F} L_{{D}_{f}}(\omega)
%\afterEquation
%\label{eq:loss_function}
%\end{equation}
%where $L_{C}(\omega)$ is the cross-entropy loss applied to samples from old and new classes, %$L_{{D}_{f}}$ is the distillation loss of the $f$ \textit{classification layer} and $F$ is the total %number of \textit{classification layers}. 
%A sketch of the incremental loss function and its connections can be seen in Fig.~\ref{fig:model-loss}a.



